Unveiling the Dreams of Word Embeddings: Towards Language-Driven Image Generation

We introduce language-driven image generation, the task of generating an image visualizing the semantic contents of a word embedding, e.g., given the word embedding of grasshopper, we generate a natural image of a grasshopper. We implement a simple method based on two mapping functions. The first takes as input a word embedding (as produced, e.g., by the word2vec toolkit) and maps it onto a high-level visual space (e.g., the space defined by one of the top layers of a Convolutional Neural Network). The second function maps this abstract visual representation to pixel space, in order to generate the target image. Several user studies suggest that the current system produces images that capture general visual properties of the concepts encoded in the word embedding, such as color or typical environment, and are sufficient to discriminate between general categories of objects.

==> sections/introduction.tex <==
\section{Introduction}
\label{sec:intro}


Main ideas from ACL-short submitted.

Some more references now on the ``real'' generation.
Brief mention that we are simimulating a generative process, so 
end-to-end integration with Language with a generative model like DRAW.

Explanation of what we are able to distringuish and what not.
Image of the category-level image in Figure~\ref{fig:summary} (need to re-draw categories vertically).

\begin{figure*}[b]
\begin{centering}
\includegraphics[scale=0.6]{figs/summary}
\end{centering}
\caption{10 generated images per category, for our 20 categories, grouped my macro-category.\label{fig:summary}}
\end{figure*}



==> sections/introduction2.tex <==
\section{Introduction}
\label{sec:introduction}



\textbf{Some questions that this visualization will help us understand, is what kind of properties do corpora encode for words. For example, i find kind of interesting that we could get the color out of the
word vector, where as in the paper with Elia you basically say that DSM are very bad with colors!}

What is the meaning of a word?
This question is very fundamendal for language sciences and in vector space, researchers  ``visualize'' how distributed/distributional semantic models encode the meaning of words through corpora 2D scatterplot illustrating the distances between a set of word representations. We propose a much more direct approach to visualization of meaning. Given a vector representing a word in a corpus-derived distributed space, we want to generate a picture depicting how the denotatum of the word looks like according to the model. Given, say, the word2vec vectors of words like \emph{ambulance}, we want to know how that ambulance looks like (see Figure \ref{fig:summary} at B-9 for the answer). Thus, we propose the task of
language-modulated image generation.

Current qualitative analysis of distributed semantic
models is limited to assessing the \emph{relation} between words,
e.g., by looking at, or plotting, nearest neighbour sets, but it lacks
methods to inspect the properties of a specific word directly. Our
image generation approach will allow researchers to ``see'', in a very
literal sense, how a model represents a single word. Moreover, in the
spirit of the ``\emph{A picture is worth a thousand words}'' adage,
the generated images will allow researchers to quickly eyeball the
results, getting the gist of what a model is capturing much faster
than from textual neighbour lists. For example, a more ``topical''
model might produce pictures depicting the wider scenes in which
objects occur (a ball being dribbled by soccer players), whereas a
model capturing strictly conceptual aspects might produce narrow views
of the denoted objects (a close-up of the ball). Image generation
could also be used to explore the effect of different input corpora on
representations: e.g., given a historical corpus, generate images for
the \emph{car} word representations induced from early 20th-century
vs.~21st-century texts. %As a last example,
%Aletras and Stevenson \cite{Aletras:Stevenson:2013} proposed to examine the topics of
%Topic Models by associating them with images retrieved from the
%Web. Given that topics are represented by vectors, we could 
%directly \emph{generate} images representing these topics.

\begin{figure*}[h]
\begin{centering}
\includegraphics[scale=0.6]{figs/summary}
\end{centering}
\caption{10 generated images per category, for our 20 categories, grouped my macro-category.\label{fig:summary}}
\end{figure*}


In cognitive science, there is a lively debate on whether abstract words have
embodied representations,
\cite{Barsalou:WiemerHastings:2005,Lakoff:Johnson:1999}, an issue that has
recently attracted the attention of the distributed semantics community
\cite{Hill:Korhonen:2014b,Kiela:etal:2014,Lazaridou:etal:2015b}. An intriguing
application of image generation would be to produce and assess imagery for
abstract concepts. Recent work in neuroscience attempts to generate images of
``what people think'', as encoded in vector-based representations of fMRI
patterns~\cite{Naselaris:etal:2009,Nishimoto:etal:2011}. Our method could then
provide a way to assess corpus-based word representations in terms of whether
the imagery they produce resembles that of humans thinking of the same words.

In the long term, we would like to move beyond words, towards generating images
depicting the meaning of phrases and sentences. This would nicely complement
current work on generating verbal descriptions of
images~\cite{Karpaty:FeiFei:2014,Kiros:etal:2014b} with the inverse task of
generating images from verbal descriptions.

Generating images from vectorial word representations is of course extremely
challenging. However, various relevant strands of research have reached a level
of maturity that makes it a realistic goal to pursue. First, tools such as
word2vec \cite{Mikolov:etal:2013b} and Glove \cite{Pennington:etal:2014}
produce high-quality word representations, making us confident that we are not
trying to generate visual signals from semantic noise. Second, there is very
promising recent work on learning to map between word representations and an
(abstract) image space, for applications such as image retrieval and annotation
\cite{Frome:etal:2013,Karpaty:FeiFei:2014,Kiros:etal:2014b,Lazaridou:etal:2014,Socher:etal:2014}.
Finally, the computer vision community is starting to explore more actively the
task of image generation~\cite{Gregor:etal:2015}, typically in an attempt to
understand the inner workings of visual feature extraction
algorithms~\cite{Zeiler:Fergus:2014}. \textbf{Here I should probably mention
classic papers on image generation with generative models, that are not
language modulated?}

The main aim of this paper is to introduce the task of language-modulated image
generation and assess its current feasibility, given state-of-the-art word
representation, cross-modality mapping and feature inversion methods. Briefly,
our proposed pipeline works as follows.  Our input is given by pre-computed
word representations (word2vec). This input  is then ``translated''
 to a visual representation, by using a \emph{cross-modal mapping} method, 
that learns to map word representations to visual representations in
a high-level visual feature space (specifically, we use activations from
different layers of convolutional neural network as high-level image
representations). Finally, this visual representation is \emph{inverted} 
to produce an image. 

Importantly, we apply this generation method to words and their images that are
neither used to train the cross-modal mapping function, nor used to learn the
feature inversion function.  So, for example, our system had to map
\emph{ambulance} onto visual space without having ever been exposed to labeled
ambulance images, and it generated the
\emph{ambulance} image without knowing how they look like (\emph{zero-shot} setting).



==> sections/introduction3.tex <==
\section{Introduction}
\label{sec:introduction}

Recent work (for example, \cite{Karpaty:FeiFei:2014,Kiros:etal:2014b})
has introduced effective methods to generate linguistic descriptions
of the contents of a given image. In this paper, we take a first step
towards the symmetric goal of generating an image to visualize the
contents of a linguistic message -- more precisely, we introduce a
method to generate pictures from words. We refer to our new task as
\emph{word-driven image generation}.

Word-driven image generation can serve as an evaluation tool providing
intuitive visualization of what computational representations of word
meaning encode. More ambitiously, effective word-driven image
generation could complement image search and retrieval, producing
images for words that are not associated to images in a certain
collection, either for sparsity, or due to their inherent properties
(e.g., artists and psychologists might be interested in images of
abstract words). Generating images for single words is also the first
step towards generating images depicting the meaning of phrases and
sentences, a task on which direct image retrieval will always suffer
of chronic sparseness issues.

To perform word-driven image generation, we combine various recent
strands of research.  Tools such as word2vec \cite{Mikolov:etal:2013b}
and Glove \cite{Pennington:etal:2014} have been shown to produce
extremely high-quality vector-based word representations, or
\emph{word embeddings}. At the same time, in computer vision, images
are effectively represented by vectors of abstract visual features,
such as those extracted by Convolutional Neural Networks (CNNs)
\cite{Szegedy:etal:2014}. Consequently, the problem of translating
between linguistic and visual representations has been coached in
terms of learning a \emph{cross-modal mapping} function between vector
spaces
\cite{Frome:etal:2013,Lazaridou:etal:2014,Socher:etal:2013a}. Finally,
recent work in computer vision, motivated by the desire to achieve a
better understanding of what the layers of CNNs and other deep
architectures have really learned, has proposed \emph{feature
  inversion} techniques that map a representation in abstract visual
feature space (e.g., from the top layer of a CNN) back onto pixel
space, to produce an actual image
\cite{Gregor:etal:2015,Zeiler:Fergus:2014}.

Our word-driven image generation system takes a word embedding as
input (e.g., the word2vec vector for \emph{grasshopper}), projects it
with a cross-modal function onto visual space (e.g., onto a
representation in the space defined by a CNN layer), and then applies
feature inversion to it (using the method of
\cite{Vondrick:etal:2014}) to generate an actual image (cell A18 in
Figure \ref{fig:summary}). We test our system in a rigorous
\emph{zero-shot} setup, in which words and images of tested concepts
are neither used to train cross-modal mapping, nor employed to induce
the feature inversion function. So, for example, our system mapped
\emph{grasshopper} onto visual and then pixel space without having
ever been exposed to grasshopper pictures.

Figure \ref{fig:summary} illustrates our results (``answer key'' for
the figure provided as supplementary material). While it is difficult
to discriminate among similar objects based on these images, the
figure shows that our word-driven image generation method already
captures the broad gist of different domains (food looks like food,
animals are blobs in a natural environment, and so on).

\textbf{I think toy sports in the figure should be toy/sports}

\begin{figure*}[t]
\begin{centering}
\includegraphics[scale=0.6]{figs/summary}
\end{centering}
\caption{10 random generated images per category for 20 basic
  categories, grouped my macro-category. See supplementary materials
  for the answer key.\label{fig:summary}}
\end{figure*}



==> sections/model-selection.tex <==
\subsection{Model Selection}


\paragraph{Selection of Visual Representations (Experiment 1)}
Generate image
from gold label using fc7 vs pool5 and centroid vs averaged.  For 50 words, ask
subjects which of the images generated by each of the 4 combinations they
prefer.  Collect 20 judgements per word.
\paragraph{Results} For each model, the first column reports the number of words
for which that model received most votes, the second column reports the number
of times the model received most votes AND the number of votes it received is
significantly different from chance (0.25) according to a two-tailed binomial
test, $p<0.05$. Ties (two cases) are excluded:

\begin{table}[h]
\begin{tabular}{l l l}
fc7\_centroid    & 5       & 2\\
pool5\_centroid  & 24      & 18\\
pool5\_prototype & 14      & 10\\
fc7\_prototype   & 5       & 0\\
tie     	& 2       & 0\\
\end{tabular}
\caption{Validation of image generation models}
\label{tab:exp1}
\end{table}

\paragraph{Selection of Cross-modal Mapping (Experiment 2)}
Generate image from word vectors via cross-modal mapping in 0 shot
setting using enet, ridge, lasso, plain regression.  For 50 words, ask subjects
which of the images generated by each of the 4 regression methods they prefer.
\paragraph{Results} Denotation of the table similar to experiment 1.
\begin{table}[h]
\begin{tabular}{l l l}
pool5\_centroid\_regress  &21      &9\\
pool5\_centroid\_elnet    &7       &2\\
pool5\_centroid\_ridge    &11      &4\\
pool5\_centroid\_lasso    &4       &1\\
tie     &7       &0\\
\end{tabular}
\caption{Cross-modal mapping validation}
\label{tab:exp2}
\end{table}




==> sections/related_angeliki.tex <==

\subsection{Experiment 4: Pick correct image for a label}

For each dreamed concept, we select an intruder that is its closest semantic
neighbor in the McRae space, i.e. a concept that is semantically and visually
similar to the dreamed concept. For these two concepts, we generate
two  images from the word vectors of the two concepts and then we ask
particants to judge  which of the two images is more likely to denote the
dreamed concept.

Results are summarized in Table~\ref{tab:exp4}.  Overall, performance in this
task drops dramatically compared to the results in the previous case. However,
if we consider that in the majority of the cases (379/472), dreamed concept and
intruder come from the same category, this makes the tasks really challenging.
While in the previous experiment participants were indirectly asked to identify
in the images coarse-grained properties that can that could distringuish
concepts from different categories, in this experiment there are only
fine-grained visual differences between the two concepts.  Despite that,
significant judgements in favor of the dreamed image are twice as much as in
favor of the random image.

Perhaps not surprisingly, the majority of the correct answers (30/41) come from
cases were items belong to the same category, hinting that the generation has
the potential to capture intra-category distrinctions. A manual inspection of
these cases revealed that the generation was able to capture primitive
properties of the dreamed concept related to its most prototypical environment
of the object, as for example in the case of \textit{turtle}-\textit{tortoise}
(images J-10 and I-19).  Interestingly, in some of the cases, the pairs of
concepts had very different prototypical color, and that was preserved in the
generated images, making thus the distrinction between them possible, as in in
that case the generation was able to preserve the most prototypical color, as
for example in the cases of \textit{flamingo}-\textit{partridge}  (see images
G-16 and H-16) and \textit{candle}-\textit{crayon} (see images J-10 and I-10).
  
\tb{turtle is I-20. plus I kept the order you had in the list, related
  vs. dreamed concept}

\tb{candle and crayon cannot be 10: 10 is building?}


For the cases were the random label was preferred, only 3 cases correspond to
concepts in different categories, but even in these cases, dreamed concept and
intruder share very strong visual properies (\textit{dish}-\textit{bowl},
\textit{marble}-\textit{thermometer} and \textit{parsley}-\textit{emerald}.  

Overall, while there are isolated cases in which we can indeed distringuish
between objects of the same category, this is done when there are primitive
distinctions that can be indirectly encoded in the word vector and can get
pulled out by the visual pipeline.

\begin{table}[h]
\begin{tabular}{l l }
Label           & Trials\\\hline
Correct Label  &41\\
Random Label   &22\\
\end{tabular}
\caption{Significant preference for correct/random image, same as above.}
\label{tab:exp4}
\end{table}


The question that naturally arises is what is currently the bottleneck of our
pipeline?  Is it the fact that some information is not encoded in language and
thus trivially cannot get pulled out by the inversion algorithm, or is the low
quality of the feature inversion component? Unfortunately, it turns out that it
is not easy to rule out the first hypothesis since it is not
straight-forward  to list which properties as encoded in a
word vector. For this reason, we assume perfect cross-modal mapping, and
instead we focus on assessing the quality of the feature inversion component
when applied on the real visual representations of the concepts as extracted
from images.

Again, we repeat a similar experiment as above, but this time by generating
images from visual representations.  Given a dreamed concept and its intruder,
we generate their two images and ask participants which image represents the
dreamed concept better.








\iffalse
\begin{verbatim}
RESULTS for related experiment

%CORRECT LABEL

RAFFA, please see here to tell me if the examples are ok
Users where presented with the image of CONCEPT and the image
of RELATED and were asked which one is the CONCEPT.
The url of the images are in the file exp4-results.R
GOOD from same category 
       RELATED       CONCEPT
10     asparagus     parsley  20      17
46         bison     buffalo  20      17
50        blouse       shirt  20      17
64         brush       broom  20      17
73      building  skyscraper  20      17
86       cabinet    cupboard  20      17
126       cougar         fox  20      17
131       crayon      candle  20      18 (I-10 and J-10) (different item color)
132    crocodile   alligator  20      17
152         doll         toy  20      17
162     earmuffs       parka  20      17
221         lamp  chandelier  20      17
224      leopard     giraffe  20      19
233      machete       knife  20      17
237     mandarin     pumpkin  20      19
256   motorcycle     scooter  20      18
262    nectarine       peach  20      19
273         oven   projector  20      19
288    partridge    flamingo  20      17 (H-16 and G-16) flamingos are ping!
324       python rattlesnake  20      17
351         seal     dolphin  20      18
382 sledgehammer      hammer  20      17
383 sledgehammer        rake  20      18
389      spatula       ladle  20      17
391        spear     harpoon  20      18
393      spinach   asparagus  20      18
410   strawberry   raspberry  20      19
425     tortoise      turtle  20      17  (I-19 and I-20) turtles can be water, while tortoise always land
438        trout    mackerel  20      17
450       turnip      carrot  20      17

GOOD from different category
27   barrel       pier  20      18
33  bathtub       sink  20      18
45    bison      whale  20      17 (B-20 and A-19) trivial
84  cabinet       barn  20      17
85  cabinet       shed  20      17
119    coin      baton  20      18
234 machete   scissors  20      17
240  marble      wheel  20      19
357  shield  submarine  20      17
363 shotgun helicopter  20      18 (J-7 and E-9) 
467    whip     muzzle  20      18


RANDOM LABEL
	CONCEPT    RELATED     CAT OF RELATED    CAT OF CONCEPT
3     alligator   crocodile   reptileamphibian   reptileamphibian
11    asparagus     spinach  fruitandvegetable  fruitandvegetable
47    blackbird       raven               bird               bird
51         boat        raft            vehicle            vehicle
52         boat    sailboat            vehicle            vehicle
70      buffalo       bison             mammal             mammal
76       bureau     dresser furniturelargetool furniturelargetool
79      buzzard        crow               bird               bird
149        dish        bowl          container               tool    -> both round
209         hut     cottage           building           building
241      marble thermometer               tool          toysports    -> both round
276          ox       camel             mammal             mammal
284     parsley     emerald      naturalobject  fruitandvegetable    -> both green
290       peach   nectarine  fruitandvegetable  fruitandvegetable 
327   raspberry  strawberry  fruitandvegetable  fruitandvegetable
330 rattlesnake      python   reptileamphibian   reptileamphibian
355       sheep        lamb             mammal             mammal
377       skunk       zebra             mammal             mammal
403      stereo       radio          appliance          appliance
407       stove        oven          appliance          appliance
446      turnip cauliflower  fruitandvegetable  fruitandvegetable
452      turtle    tortoise   reptileamphibian   reptileamphibian

\end{verbatim}

\fi









==> sections/upper-bound.tex <==

\subsection{Experiment 3: pick the correct image for a label (upper-bound).}

The novelty of our proposal lies on the assemble of a cross-modal
mapping module (from word vector to visual vector) and an image
generation module (from visual vector to image). We exploit
out-of-the-shelves generation module and focus on the cross-modal
mapping part and its integration within the full system.  Hence, we
can set our upper-bound by skipping the cross-modal mapping and by
starting directly from the visual-vectors which generate ``gold
standard'' images. We repeat the previous experiment by using these
``gold standard'' images (we cannot expect our image to be better than
these ones).  Given a dreamed concept and the most related one (from
the McRae space), by taking their visual vectors generate their two
images and ask which image represents the dreamed concept.

The numbe of images for which no significant preference was express is
lower than above but still quite high: 356/472.  Of the 116 images for
which a preference is given, 71.5\% (38/116) were correctly labeled
and 28.4\% (33/116) were assigned the wrong concept.


\paragraph{Results}
   Min. 1st Qu.  Median    Mean 3rd Qu.    Max.\\
 0.0500  0.4000  0.6000  0.5679  0.7500  1.0000\\

\begin{table}[h]
\begin{tabular}{l l }
Label           & Trials\\\hline
No preference & 356 \\
Correct Label  & 71.5\% (83/116)\\
Random Label   & 28.4\% (33/116)\\
\end{tabular}
\caption{Significant preference for correct/random image, same as above.}
\label{tab:exp5}
\end{table}






